Graph-based Agent Memory: Taxonomy, Techniques, and Applications

Memory emerges as the core module in the Large Language Model (LLM)-based agents for long-horizon complex tasks (e.g., multi-turn dialogue, game playing, scientific discovery), where memory can enable knowledge accumulation, iterative reasoning and self-evolution. Among diverse paradigms, graph stands out as a powerful structure for agent memory due to the intrinsic capabilities to model relational dependencies, organize hierarchical information, and support efficient retrieval. This survey presents a comprehensive review of agent memory from the graph-based perspective. First, we introduce a taxonomy of agent memory, including short-term vs. long-term memory, knowledge vs. experience memory, non-structural vs. structural memory, with an implementation view of graph-based memory. Second, according to the life cycle of agent memory, we systematically analyze the key techniques in graph-based agent memory, covering memory extraction for transforming the data into the contents, storage for organizing the data efficiently, retrieval for retrieving the relevant contents from memory to support reasoning, and evolution for updating the contents in the memory. Third, we summarize the open-sourced libraries and benchmarks that support the development and evaluation of self-evolving agent memory. We also explore diverse application scenarios. Finally, we identify critical challenges and future research directions. This survey aims to offer actionable insights to advance the development of more efficient and reliable graph-based agent memory systems. All the related resources, including research papers, open-source data, and projects, are collected for the community in https://github.com/DEEP-PolyU/Awesome-GraphMemory.

==> tex/overview.tex <==
Graph-based memory has emerged as a powerful and flexible paradigm for agent system design. By representing memory elements as nodes and their relationships as edges, graph structures naturally accommodate relational dependencies, multi-level abstraction, and temporal dynamics. This allows agents not only to store past experiences but also to reason over them, draw inferences, and adapt their behavior over time. Graph-based memory supports key agent capabilities such as personalization, hallucination mitigation, and continual self-improvement, making it a general and expressive framework for next-generation intelligent agents. 

% \section{Overview}\label{sec:overview}
This survey provides a comprehensive analysis of graph-based agent memory, systematically detailing its taxonomy, key techniques, application scenarios, and future directions. It is organized into ten main sections that progress from foundational concepts to practical implementations. Specifically, we begin in Section~\ref{sec:def} by defining the basic concepts and scope of agent memory, tracing its evolution from traditional linear paradigms to graph-structured representations, analyzing the limitations of existing memory frameworks in relational modeling and hierarchical organization, and highlighting the core advantages of graph-based memory in complex reasoning, long-term evolution, and personalized interaction. The following three sections systematically dissect the core components of graph-based memory management: memory construction methods, including representation and organization based on structures such as knowledge graphs, temporal graphs, and hypergraphs (Section~\ref{sec:storing}); memory retrieval mechanisms, covering techniques for information extraction through structure-aware, semantic embedding, and temporal reasoning approaches (Section~\ref{sec:retrieval}); and memory maintenance strategies, involving dynamic revision, compression, and fusion of memory content (Section~\ref{sec:evolving}). Moving toward practical aspects, Section~\ref{sec:opensource} reviews open-source libraries and benchmark datasets that support the development and evaluation of graph-based memory systems, offering guidance for implementation and performance assessment. Subsequently, Section~\ref{sec:applications} explores the concrete applications and effectiveness of graph-based memory across various domains, including conversational systems, financial agents, game agents, robotics, and scientific agents. Finally, Section~\ref{sec:limitations} and Section~\ref{sec:conclusion} conclude the survey by identifying critical challenges in scalability, privacy, security, and cross-domain transfer, and outlining promising future research directions. 

Throughout, this survey balances fundamental concepts, state-of-the-art methods, and practical applications, aiming to serve as a systematic reference for researchers advancing memory system innovations and for practitioners selecting appropriate graph-based memory structures and techniques for specific scenarios. All related resources, including publications, open-source data, and projects, are collected for the community in \textcolor{blue}{\url{https://github.com/DEEP-PolyU/Awesome-GraphMemory.git}}.
% This survey provides a systematic review of the state-of-the-art in graph-based agent memory. We begin by introducing a hierarchical taxonomy that categorizes existing graph memory architectures, such as knowledge graphs, temporal graphs, hypergraphs, and hybrid structures, and detail their structural characteristics, design principles, and representative implementations. We then systematically analyze the core memory management techniques, including methods for memory construction, retrieval, and updating, which are critical for maintaining scalable and usable memory systems. To support practical development and evaluation, we also summarize available open-source libraries and benchmarks tailored for self-evolving graph-based memory. Furthermore, we explore diverse application scenarios, including conversational agents, financial systems, game agents, robotics, and scientific discovery, where graph memory has demonstrated a significant impact or holds promising potential. Finally, we discuss key challenges and future directions, addressing issues such as scalability, privacy, and cross-domain transferability. 

% The remainder of this survey is organized as follows: Section 3 situates graph-based agent memory within the broader landscape of agent memory paradigms. Sections 4, 5, and 6 delve into memory management techniques, available resources, and applications, respectively. Section 7 outlines limitations and promising research avenues, and Section 8 concludes. All the related resources, including research papers, open-source data, and projects, are collected for the community in \textcolor{blue}{\url{https://github.com/DEEP-PolyU/Awesome-GraphMemory}}.
